Lower Bounds on Adversarial Robustness from Optimal Transport

While progress has been made in understanding the robustness of machine learning classifiers to test-time adversaries (evasion attacks), fundamental questions remain unresolved. In this paper, we use optimal transport to characterize the minimum possible loss in an adversarial classification scenario. In this setting, an adversary receives a random labeled example from one of two classes, perturbs the example subject to a neighborhood constraint, and presents the modified example to the classifier. We define an appropriate cost function such that the minimum transportation cost between the distributions of the two classes determines the minimum $0-1$ loss for any classifier. When the classifier comes from a restricted hypothesis class, the optimal transportation cost provides a lower bound. We apply our framework to the case of Gaussian data with norm-bounded adversaries and explicitly show matching bounds for the classification and transport problems as well as the optimality of linear classifiers. We also characterize the sample complexity of learning in this setting, deriving and extending previously known results as a special case. Finally, we use our framework to study the gap between the optimal classification performance possible and that currently achieved by state-of-the-art robustly trained neural networks for datasets of interest, namely, MNIST, Fashion MNIST and CIFAR-10.

==> sections/extra.tex <==
\bcomment{
\paragraph{Total variation and adversarial optimal transport cost}
The optimal transportation costs $C_N(P_X,P_{\tilde{X}})$ are closely connected to total variation distance.
Observe that when we follow the convention $\infty \cdot 0 = 0$,
\[
  c_N = (\infty \cdot c_N) \circ c_{\text{TV}}.
\]
If $c_N(x,\tlx) = 0$, then we have $c_N(x,\tlx) = \infty \cdot c_N(x,\tlx) + c_{\text{TV}}(\tlx,\tlx)$.
  If $c_N(x,\tlx) = 1$, then for any $\tlx' \in N(x)$, we have $c_N(x,\tlx) = \infty \cdot c_N(x,\tlx') + c_{\text{TV}}(\tlx',\tlx)$.

Let $\Pi_N(P_{X},P_{Y})$ be the set of couplings $P_{XY}$ of $P_X$ and $P_Y$ such that $P_{XY}(Y \in N(X)) = 1$.
Let $\mcN_N$ be the set of probability distributions $P_{\tilde{X}}$ on $\tilde{\mcX}$ such that $C_N(P_X,P_{\tilde{X}}) = 0$.
\begin{lemma}
  \[
    \inf_{P_{X \tilde{X}} \in \Pi(P_{X},P_{\tilde{X}})} \E[c_N(X,\tilde{X})] = \inf \{C_{\text{TV}}(P',\tilde{P}) : \exists P_{X \tilde{X}} \in \Pi(P_{X},P_{\tilde{X}}) : \E[c_N(X,\tilde{X})] = 0\}
  \]
  \[
    C_N(P_X,P_{\tilde{X}}) = \inf_{P_{\tilde{X}'} \in \mcN_N(P_X)} C_{\text{TV}}(P_{\tilde{X}'},P_{\tilde{X}})
  \]
\end{lemma}

\[
  (P \wedge Q)(S) = \inf_{T \subseteq S} P(T) + Q(S \setminus T)
\]


%Kantorovich duality relates the two standard definitions of total variation distance:
%\[
%  \sup_A \mu(A) - \nu(A) = \int_{\mcX} 
%\]
%If we take $\mcX = \mcY$ and take $N(x) = \{x\}$ for all $x \in \mcX$, then our adversary becomes trivial and we obtain the standard supervised classification problem.
}


\bcomment{
\begin{definition}
  For $U \subseteq \tilde{\mcX}$, let the adversarial interior of $U$ be
  \[
    \interior_N (U) = \{x \in \mcX : N(x) \subseteq U\}.
  \]

\end{definition}
The other two are $\interior_N(h^{-1}(1))$ and $\interior_N(h^{-1}(-1))$.
Observe that
\[
  \one[x \in \interior_N(h^{-1}(1))] + \one[y \in \interior_N(h^{-1}(-1))] \leq c(x,y) + 1.
\]
}

\bcomment{
  \begin{lemma}
  Let $h : \tilde{\mcX} \to \{-1,1\}$.
  The performance of
  \[
    P_1(\interior_N(h^{-1}(1))) + P_{-1}(\interior_N(h^{-1}(-1)))
  \]
\end{lemma}


\begin{definition}
  \begin{align*}
    f_1,f_{-1} : \mcX \to \R &\text{ s.t. } \forall x,y \in \mcX,  f_1(x) + f_{-1}(y) \leq c(x,y)\\
    S_1, S_{-1} \subseteq \mcX &\text{ s.t. } c(S_1,S_{-1}) = 1\\
    h : \tilde{\mcX} \to \{-1,1\} &
  \end{align*}

  \begin{align*}
    &\eq \sup_{f_1,f_{-1}} E_1[f_1(X)] + E_1[f_{-1}(X)]\\
    &= \sup_{S_1,S_{-1}} P_1(S_1) + P_{-1}(S_{-1})\\
    &= \sup_h P_1(\interior_N(h^{-1}(1))) + P_{-1}(\interior_N(h^{-1}(-1)))
  \end{align*}
  
\end{definition}
}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

